CLASS: A Design Framework for building Intelligent Tutoring Systems based on Learning Science principles

We present a design framework called Conversational Learning with Analytical Step-by-Step Strategies (CLASS) for building advanced Intelligent Tutoring Systems (ITS) powered by high-performance Large Language Models (LLMs). The CLASS framework empowers ITS with two key capabilities. First, through a carefully curated scaffolding dataset, CLASS equips ITS with essential problem-solving strategies, enabling it to provide tutor-like, step-by-step guidance to students. Second, by using a dynamic conversational dataset, CLASS assists ITS in facilitating natural language interactions, fostering engaging student-tutor conversations. The CLASS framework also provides valuable insights into ITS' internal decision-making process which allows seamless integration of user feedback, thus enabling continuous refinement and improvement. We also present a proof-of-concept ITS, referred to as SPOCK, which is trained using the CLASS framework with a focus on introductory college-level biology content. A carefully constructed protocol was developed for SPOCK's preliminary evaluation, examining aspects such as the factual accuracy and relevance of its responses. Experts in the field of biology offered favorable remarks, particularly highlighting SPOCK's capability to break down questions into manageable subproblems and provide encouraging responses to students. Code and models are available at https://github.com/luffycodes/Tutorbot-Spock.

==> sections/design_v3.tex <==
The design framework for our Tutorbot is centered around the construction of two datasets and an automatic feedback mechanism for continuous fine-tuning of the Tutorbot model.
In this section, we describe the rationale behind the framework, delve into the organization of the datasets, and outline the methodology for training the Tutorbot using these datasets.

\subsection{First Dataset: Problem Creation, Subproblems, and Feedback}

The first dataset encompasses challenging problems specifically designed for the subject of Biology, along with their corresponding subproblems, essential facts for solving the main problem, hints, incorrect student responses, and relevant feedback for each subproblem. 
This comprehensive set of elements, especially with the focus on breaking down problems into manageable subproblems, aims to equip the Tutorbot with crucial skills to provide step-by-step assistance to learners, promoting deeper understanding and engagement with the subject matter.

In constructing this dataset, we employed the following prompt that outlines the requirements necessary for generating content:

\begin{itemize}
  \item Generate a hard, challenging problem for a given section and learning objective.
  \item Provide facts necessary to answer the main problem.
  \item Break down the main problem into subproblems.
  \item Present the final solution to the main problem.
  \item For each subproblem, generate a hint, one incorrect student response, and corresponding feedback.
\end{itemize}

The output is organized in a JSON structure, which includes the main problem, subproblems, facts, and solution, along with hints, incorrect responses, and feedback for each subproblem.
The prompt and an example is included in Appendix~\ref{app:p1} and ~\ref{app:e1} respectively.

As the first dataset equips the Tutorbot with essential problem-solving skills, such as providing hints and segmenting problems into smaller tasks, it paves the way for the application of these capabilities through the second dataset. 
In the following section, we will explore the creation of the second dataset, which focuses on engaging and cohesive student-Tutorbot.

\subsection{Second Dataset: Simulated Conversations}
After being trained on the first dataset, the Tutorbot acquires essential techniques such as generating hints, providing feedback, and breaking problems into smaller tasks, thus ensuring efficient guidance for students in their learning journey.
However, to effectively teach the Tutorbot how to apply these skills seamlessly within real-time conversations, a second and even more crucial dataset is needed.

This second dataset contains simulated conversations between students and the Tutorbot revolving around specific questions, allowing the Tutorbot to practice decomposing main problems into subproblems and assisting students in sequentially solving each part.
By training the Tutorbot using this vital second dataset, it becomes adept at applying the foundational skills acquired from the first dataset during ongoing conversations and adapting its guidance as necessary.

To generate these comprehensive and interactive conversations, the following prompt is employed:

\begin{itemize}
  \item Create a mock conversation between a student and a Tutorbot, an AI-powered chatbot designed to help students with a specific question.
  \item The conversation should focus on breaking down the main problem into subproblems and guiding the student to solve each subproblem sequentially.
  \item The Tutorbot should provide hints and address different types of student responses, including incorrect, partially correct, and ambiguous answers.
  \item Simulate many incorrect responses from the student to test the Tutorbot's ability to handle various scenarios.
  \item Use a JSON structure to represent the conversation, including the student's response, the Tutorbot's decision, the subproblem being solved, and the Tutorbot's reply.
\end{itemize}

The prompt and an example is included in Appendix~\ref{app:p2} and ~\ref{app:e2} respectively.

\subsubsection{Tutorbot's Response Template in Mock Conversations and Model Refinement}
\label{sec:decision}

A pivotal aspect of our design framework rests in the implementation of a fixed response template for the Tutorbot during the mock conversations. 
This structured template ensures consistency and coherence in its responses as it engages in simulated conversations with students.
Centered around the Tutorbot's thought process and decision-making, the response template presents a systematic approach for addressing various types of student responses and inquiries.

The output JSON for the Tutorbot's response comprises the following components:

\begin{itemize}
  \item \textbf{Thoughts of Tutorbot}: Represents the decision-making process and evaluation of the student's response.
  \item \textbf{Evaluation of Student Response}: Categorized as a, b, c, d, e, f, or g, indicating the type of student response (e.g., incorrect, partially correct, ambiguous, etc.).
  \item \textbf{Action Based on Evaluation}: Numerical codes representing the appropriate action for the Tutorbot in response to the student, such as providing hints, feedback, clarification, or solutions.
  \item \textbf{Subproblem State}: Designated by w, x, y, or z, describing the current state of the subproblem being tackled (e.g., ongoing, finished, moving to the next subproblem, etc.).
  \item \textbf{Subproblem}: Specifies the current subproblem that the student must solve.
  \item \textbf{Tutorbot}: Contains the actual response text from the Tutorbot that engages with the student and provides guidance.
\end{itemize}

By employing this fixed response template, the Tutorbot maintains a consistent and structured approach in handling various student responses and remains focused on guiding them through the problem-solving process.
Furthermore, using this response template enables better explainability of the Tutorbot's decision-making.
It offers insights into the rationale behind the model's choices, such as the evaluation of student responses and the subsequent actions it takes.

Here is an example of a response from the Tutorbot, showcasing how the response looks like when using the fixed response template:

\begin{lstlisting}
{
   ""Student"": ""DNA is a double helix made of sugar, phosphate, and bases."",
   ""Thoughts of Tutorbot"": ""The student's answer is partially correct."",
   ""Evaluation of Student Response"": ""c"",
   ""Action Based on Evaluation"": ""4"",
   ""Subproblem State"": ""x"",
   ""Subproblem"": ""Understanding the structure of DNA"",
   ""Tutorbot"": ""That's partially correct. DNA is a double helix, but it's important to know the four bases that make up the structure. Can you tell me the names of the four bases?"",
}

\end{lstlisting}

\subsubsection{Utilizing the Response Template for Model Refinement}
\label{sec:refinement}

The fixed response template not only provides structure and consistency in the Tutorbot's interactions with students but also serves as a valuable tool for refining and improving the model's performance. 
By leveraging the template's components such as evaluation categories, numeric action codes, and subproblem states, we can create a loss function that quantifies potential errors and inaccuracies in the Tutorbot's responses.

This iterative refinement approach ensures that the Tutorbot remains informed by real-world student interactions and steadily enhances its problem-solving and conversational capabilities. 
It enables the model to evolve continually, becoming more accurate and effective in providing step-by-step guidance.

In conclusion, it is crucial to emphasize the synergistic relationship between the first and second datasets in the design framework of our Tutorbot.
The first dataset lays the groundwork by providing the Tutorbot with problem-solving strategies, hints, and feedback mechanisms for various subproblems.
On this foundation, the second dataset, primarily through its fixed response template, applies the acquired skills to create a more engaging and personalized learning experience for students, expertly addressing various types of student responses and inquiries during simulated conversations. 
Furthermore, the response template presents a unique advantage by offering a loss function, which enables continuous model improvement and increased explainability, ultimately leading to a more efficient and effective AI-driven educational tool.

\subsection{Indexed Search Over Biology Textbooks: A Robust Approach to Maximize Tutorbot Response Relevance and Minimize Hallucinations}

To further enhance the accuracy and relevancy of the Tutorbot's responses, we employ an indexed search over 60 biology textbooks as an additional verification method and a means to reduce hallucinations.
By indexing the paragraphs within the textbook, we can fetch relevant passages that correspond to the main problems and subproblems encountered during the simulated conversations.
This approach not only ensures that the Tutorbot's responses are factually correct but also aids in providing contextually relevant and helpful hints to students when they are stuck.

The indexing process begins with preprocessing the biology textbook, which includes tokenizing and cleaning the text and extracting relevant paragraphs and sections.
Next, the textbook content is indexed to create an efficient search structure, allowing for fast retrieval of relevant passages based on the input query, such as a problem or subproblem field derived from the response template. 
The integration of the indexed search mechanism with the Tutorbot's response template empowers the Tutorbot to fetch relevant passages from the textbook when generating hints or providing feedback, ensuring that its responses are both factually accurate and contextually suitable.
This approach adds an additional layer of validation to the Tutorbot's responses, contributing to an enriched learning experience for students.


==> sections/future_work.tex <==
We have identified various opportunities to enhance the proposed \fw framework.
A key priority for future updates is to address the challenge of maintaining factual accuracy in the information generated by \itsns.
LLMs are prone to occasional inaccuracies and hallucinations, and these limitations are also inherited by any \its built upon LLMs.
To mitigate these issues, we have implemented indexed search over the educational content which significantly reduced concerns regarding factual accuracy.
However, we acknowledge that additional creative guardrails are needed to further improve the accuracy of the returned information in future iterations of \fw powered \itsns.
Additionally, we only conducted a preliminary evaluation so far, which only include interactions between \its and biology domain expert.
In the next stage, we will modify \its to address the concerns of biology-learning students, followed by use \its in a small classroom to perform more comprehensive and practical evaluations, and ultimately test the tool in the real world.
The key to investigating the impact of using \its will be to see how students perform on a content assessment with and without its use. 
After a small scale evaluation, we will evaluate the impact of \its on a large scale research infrastructure.

==> sections/introduction_old.tex <==
% The emergence of chat-based Large Language Models (LLMs), such as ChatGPT and other GPT-based models \cite{gpt4sparkai,openai2023gpt4}, has significantly impacted the field of education, resulting in innovative tools and methods that enhance the learning experience \cite{kasneci2023chatgpt}.
% These advancements have led to various applications for both students and instructors, including personalized learning, support for students with disabilities, assessment generation, and lesson planning.
% Among these advancements, integrating artificial intelligence (AI) in the form of \longits (\itsns) has gained considerable attention for its potential to provide personalized, accessible, and interactive learning support.
% However, designing and implementing effective \its remains a challenge, particularly in addressing students' diverse learning needs and promoting a deeper understanding of complex concepts. 
% This highlights the need to develop innovative frameworks that leverage the power of LLMs, pushing the potential of \its to benefit students across various grade levels.

\longits (\itsns) have a history of offering valuable support to students and educators, with successful implementations such as the Cognitive Tutors in mathematics \cite{anderson1995cognitive} and the AutoTutor for computer literacy \cite{graesser2004autotutor}.
Drawing on the potential of recent advancements in natural language processing, chat-based Large Language Models (LLMs) such as ChatGPT and other GPT-based models \cite{gpt4sparkai,openai2023gpt4} present an opportunity to further revolutionize and enhance ITS by incorporating critical learning science principles.

Learning science principles are essential in understanding the cognitive processes of learners, providing personalized support, and fostering engaging learning experiences
\cite{wing2006computational, shute2017demystifying}.
By intertwining LLMs with these principles, we can ensure that ITS not only offer accurate answers but also stimulate deep learning and comprehension of complex concepts.

\iffalse
\longits (\itsns) have a history of offering valuable support to students and educators, with successful implementations such as the Cognitive Tutors in mathematics \cite{anderson1995cognitive} and the AutoTutor for computer literacy \cite{graesser2004autotutor}.
However, the development of effective ITS remains a challenge, particularly in addressing the diverse learning needs of students and promoting a deeper understanding of complex concepts.
Drawing on the potential of recent advancements in natural language processing, Large Language Models (LLMs) such as ChatGPT \cite{gpt4sparkai,openai2023gpt4} present an opportunity to overcome the challenge and enhance ITS design by incorporating learning science principles. 
Learning science principles are essential in understanding the cognitive processes of learners, providing personalized support, and fostering engaging learning experiences
\cite{wing2006computational, shute2017demystifying}.
By intertwining LLMs with these principles, we can ensure that ITS not only offer accurate and personalized answers but also stimulate deep learning and comprehension of complex concepts.
\fi

% In this study, we present a novel design framework called \longfw (\fwns) that seamlessly integrates learning science principles utilizes LLMs for building \itsns.
In this study, we present a novel design framework called \longfw (\fwns) which applies learning science principles to create an effective LLM-based ITS.
\fw aims to provide learners with thorough scaffolded step-by-step support, addressing their queries and rectifying misconceptions.
As a proof of concept to demonstrate the practicality and effectiveness of \fw  framework, we develop a Biology \its referred to as \botnamens.
Biology is chosen as a representative example due to the subject's inherent complexity and the need for students to grasp intricate concepts.

\input{figures/tutorbot}

The core objective of the \fw framework is to equip \botname with two critical capabilities: 1) providing tutor-like step-by-step guidance that fosters a deeper understanding and significantly augments students' learning experience and 2) engaging in tutor-like conversations using natural language suitable for students, ensuring conversational fluidity and adaptability. 
To achieve these capabilities, \fw implements an innovative, dual-faceted approach that utilizes two distinct training datasets.
These datasets are specifically curated to instill the desired capabilities in \botnamens, thereby leveraging the datasets as a solution for fulfilling \fwns's core objective.
\fwns's approach of utilizing the two training datasets, each to addressing a specific aspect of \botnamens's functionality is illustrated in Figure~\ref{fig:tutorbot}.
 
The first dataset, referred to as the \emph{``scaffolding dataset''} lays the foundation for equipping \botname with essential skills necessary to effectively guide students through the learning process.
The scaffolding dataset, generated using GPT-4 \cite{gpt4sparkai}, covers a wide range of components, such as problems along with their related subproblems, hints to provide guidance, solutions that are incorrect, and customized feedback for the incorrect solutions.
By endowing \botname with a holistic understanding of problem-solving strategies and methods for addressing misconceptions, the scaffolding dataset ensures the system's effective performance during interactions with students.

Building on the foundation established by the scaffolding dataset, the second \emph{``conversational dataset''} focuses on simulated conversational student-tutor interactions. 
The conversational dataset, also generated by GPT-4, consists of simulated student-tutor conversations that involve the application of problem-solving strategies acquired from the first dataset within structured, question-focused exchanges. 
Training on this conversational dataset enhances \botnamens's ability to effectively apply the skills learned in the scaffolding dataset during real-time interactions with students, providing guidance in decomposing the main problem into smaller tasks and assisting learners in solving these tasks sequentially through hints and direction.

Within the interactions contained in the second dataset, a pre-defined response template is employed to ensure consistency and coherence in \botnamens's responses.
This template addresses various situations, such as handling incorrect, correct, and ambiguous responses, as well as guiding students through subproblems and effectively addressing their inquiries.
By adhering to this template, \botname benefits from a structured approach that enables the seamless incorporation of user feedback, promoting system enhancement and fine-tuning. 
Additionally, this method offers valuable insights into the internal decision-making mechanisms of \botnamens, contributing to its continuous improvement and refinement.

% \zw{this last sentence is not entirely clear to me at this point, i.e., why this method offers valuable insights into the internal decision making mechanism of spock, the last three paragraphs could be consolidated into either 1) one paragraph focusing on experiments and insights or 2) one paragraph on the evaluation protocol, if this is novel and worthy of highlighting, and one paragraph on the results and insights} + 1 DBM

Our contributions can be summarized as follows:
\begin{enumerate}
  \setlength\itemsep{0em}
    \item We introduce a novel \longfw (\fwns) framework for building \itsns. \fw uses two synthetic datasets - the first scaffolding dataset facilitates tutor-like, step-by-step guidance, while the second conversational dataset promotes engaging interactions with learners.

    \item Under the \fw framework, we present \botnamens, a proof-of-concept \its system designed for a college-level biology course.

    \item We also develop a comprehensive evaluation protocol for \its and conduct preliminary human evaluations of \botname with biology domain experts, providing valuable insights into the effectiveness of \botnamens.

    \item We develop a thoughtfully designed response template for \botname to ensure consistency and clarity in its responses, while also providing valuable insights into \botnamens's internal decision-making process.
\end{enumerate}



% Old contributions:
% \begin{enumerate}
%     \item We introduce a novel \longfw (\fwns) framework for constructing \longits (\itsns), focusing on two primary goals: facilitating tutor-like, step-by-step guidance and promoting engaging interactions with students. 
%     The \fw framework incorporates two unique synthetic datasets generated using GPT-4 with specially crafted prompts, working together to enable the achievement of our goals.
%     The first, the scaffolding dataset, cultivates essential skills such as providing hints, feedback, and segmenting problems into smaller tasks. The second, the conversational dataset, facilitates the effective application of these acquired skills, enabling \its to engage in cohesive and interactive dialogues with learners.

%     \item Under the \fw framework, we present \botnamens, a proof-of-concept \its system designed for a college-level introductory biology course, which showcases \fwns's capabilities. \botname is trained on the scaffolding and conversational datasets, generated using GPT-4, allowing it to deliver tailored support through engaging, interactive conversations.

%     \item We develop a thoughtfully designed response template for \botname to ensure consistency and clarity in its responses. This template enables users to offer feedback on \botnamens's decisions while providing valuable insights into \botnamens's internal decision-making process.

%     \item We use an application of indexed search over educational course materials to ensure factual correctness and relevancy of \botnamens's responses, by fetching relevant passages for problems and subproblems.

%     \item We also develop a comprehensive evaluation protocol and conduct preliminary human evaluations of \botname with biology domain experts, providing valuable insights into the effectiveness of \botnamens.
% \end{enumerate}
